PARSEC V2.0: Stellar tracks and isochrones of low and intermediate mass stars with rotation

We present a new comprehensive collection of stellar evolutionary tracks and isochrones for rotating low- and intermediate-mass stars assembled with the updated version of PARSEC V2.0. This version includes our recent calibration of the extra mixing from overshooting and rotation, as well as several improvements in nuclear reaction network, treatment of convective zones, mass loss and other physical input parameters. The initial mass of the stellar models covers the range from 0.09 $M_\odot$ to 14 $M_\odot$, for six sets of initial metallicity, from Z=0.004 to Z=0.017. Rotation is considered for stars above $\sim 1 M_\odot$ with a smooth transition between non rotating and extremely fast-rotating models, based on the initial mass. For stars more massive than $\sim 1.3~M_\odot$ the full rotation range, from low to the critical one, is considered. We adopt the solar-scaled chemical mixture by Caffau et al. with Z$_\odot$ = 0.01524. All the evolutionary phases from the pre-main-sequence to the first few thermal-pulses on the asymptotic-giant-branch or central C exhaustion, are considered. The corresponding theoretical isochrones are further derived with TRILEGAL code and are converted in several photometric systems, taking into account different inclination angles. Besides magnitudes, they also offer many other stellar observables in line with the data that are being provided by current large surveys. The new collection is fully integrated in a user friendly WEB interface for the benefit of easily performing stellar population studies.

==> Answer2referee.tex <==
Title: PARSEC V2.0: Stellar tracks and isochrones of low and intermediate mass stars with rotation


AUTHORS: We thank the referee for thoughtful comments and constructive feedback. We have highlighted in bold face the changes in the manuscript.
In the following, detailed comments are given.


REFEREE: Although the physics of their rotating models has already been described in published paper (Costa et al 2019), in order to make the paper more self-explanatory, I would encourage the author to add a paragraph reminding the equations used for computing the angular momentum transport as well as the chemical element transport (equations and expressions for the different diffusion coefficient and U). Actually, rotating models computed by different authors include very different physics or even for a given physics very different numerical process for describing it. Since the present paper is focused on tracks with rotation, this is in my view important that this part be presented in the paper.

AUTHORS: We thank the referee for this thoughtful suggestion. In Section. 2.5, we have briefly added how we treat angular momentum transport in PARSEC.
    

REFEREE: Looking at the paper by Costa et al. 2019, I note that for the transport of the angular momentum by meridional currents they use a diffusive equation with a diffusion coefficient equal to abs(rU)^2/(30 Dh) and they refer to Zahn (1992). May be here it would be fair to indicate that in Zahn (1992), the angular momentum transport is treated by an advective equation (not a diffusive one, see Eq 2.7 in Zahn 1992) and that the diffusion coefficient that the authors use is actually a diffusion coefficient that was proposed in the paper by Chaboyer and Zahn (1992) for the transport of the chemical species, not the angular momentum. This is in my view important since the diffusion coefficient abs(rU)^2/(30 Dh) actually accounts for the net effect of the meridional current and of the strong horizontal diffusion for the chemical species. A big difference between chemical species and angular momentum is that the angular momentum that is transported depends on the distance to the rotation axis. Thus if a blob is mixed up along the rotation axis or in the equatorial plane, it will not make any difference for the chemical species but be different for the angular momentum. It might be fair that the authors comment on those points. Of course,  I understand that treating the angular momentum transport by meridional current need that the author provide a diffusion coefficient and the one that they use might be a possibility, but it would be fair that the limitations of this approach are at least briefly mentioned.
    
AUTHORS: We thank the referee for making this point and for the detailed explanation of the diffusion coefficient of the meridional circulation, Dmc. We agree with the referee and added the Chaboyer and Zahn (1992) reference. We made this specific choice for the sake of simplicity. Some authors, like Heger et al. (2000), define the diffusion coefficient as the product of the circulation velocity and the typical circulation length scale. Others, like Chieffi & Limongi (2013) use the Chaboyer & Zahn (1992) Dmc. also for the angular momentum transport (when they use the diffusive scheme). We decided to adopt the latter approach.
We have updated the manuscript, specifying that we use the Chaboyer & Zahn (1992) diffusion coefficient for the meridional circulation also for the transport of angular momentum. In future PARSEC release we already planned to include the full advective-diffusive equation for the momentum transport.



REFEREE: Since those models present rotating models, it would be interesting to have at least a plot showing the internal distribution of the angular velocity during the MS, subgiant and red giant phase. Another possibility would be to show for a given initial mass the evolution as a function of time during the MS phase of the central angular velocity to the surface one.  This kind of information is interesting now that helio- and asteroseismology can give access to that information.
    
AUTHORS: The authors thank the referee for his suggestion. We have added a plot (Figure 9) of the inner angular velocity profile of a 1.44 Msun star (with Z=0.014) for three given phases: i) during the MS (central hydrogen ~ 0.3); ii) at the base of the RGB phase; iii) near the RGB's tip with (log L ~ 3.35).


    
REFEREE: The authors write at the beginning of section 2.1

However, later, Asplund et al. (2006, 2009) claimed lower
values, Zsun = 0.0122 and Zsun = 0.0134, respectively. Recent
solar wind measurements give Zsun = 0.0196 +/- 0.0014 (von
Steiger & Zurbuchen 2016), however, the solar model computed
with this new abundance has been claimed to be
in disagreement with helioseismic measurements (Vagnozzi
2019).

It is not clear according to that sentence which solar model has been claimed in disagreemet with helioseismic measurements.  It seems to me (but the authors can correct me) that the low values of Z produce solar models in disagreement with helioseismic measurement not those with the classical Z=0.02 value, as I would understand from the above sentence. Can the authors clarify that point?


AUTHORS: We agree with the referee that the sentence could not be clear enough. The new value from von Steiger & Zurbuchen 2016 (Zsun = 0.0196) agrees better with helioseismology only for the sound speed at the bottom of the convective envelope and the convective zone. However, the predictions for the sound speed near the core, the surface helium abundance, and neutrino fluxes are still very discrepant with the helioseismologic measurements, as found by Vagnozzi 2019. However, we decided to remove the sentence because it was a source of confusion.



    
REFEREE: May be I missed the point but are the authors considering a metallicity dependence of the mass loss rates? Might be fair to add this information in case it is indeed missing in the present version of the paper.
    
AUTHORS: For the intermediate-mass stars we use the deJager et al. (1998) prescription corrected with a metallicity dependence as shown in Chen et al. 2015. Indeed, we added a sentence in section 2.6, to specify this information.
    
    
    
REFEREE: In Equation 5, are the authors considering a value of Gamma_e that is constant over the stellar surface (no change with the colatitude?). Such a dependence might be present due to the von Zeipel theorem as explained e.g. in Maeder & Meynet (2000). But such a dependence might only be important for very fast rotating models and thus a constant value may be adequate most of the time.
    
AUTHORS: Yes, in this work we assume that Gamma_e is constant on the surface. We update the text saying that. In a future work, we will include the dependence on the angular velocity following Maeder & Meynet (2000).


REFEREE: Is the pressure scale height estimated at the Schwarschild boundary?
    
AUTHORS: We treat the overshooting with the ballistic approximation by Bressan (1981). The pressure scale height is estimated across the convective border, and the overshooting parameter is the maximum path of a rising/sinking bubble can travel before dissolving in Hp units (across the border). The parameter is in pressure scale heights.


AUTHORS: We have updated the manuscript with all the minor points suggested by the referee in the pdf.
